Understanding Quality of Experiences on Different Mobile Browsers: Measurements, Analysis, and Implications

The web browser is one of the major channels to access the Internet on mobile devices. Based on the smartphone usage logs from millions of real-world Android users, it is interesting to find that about 38% users have more than one browser on their devices. However, it is unclear whether the quality of browsing experiences are different when visiting the same webpage on different browsers. In this paper, we collect 3-week consecutive traces of 337 popular webpages on three popular mobile browsers: Chrome, Firefox, and Opera. We first use a list of metrics and conduct an empirical study to measure the differences of these metrics on different browsers. Then, we explore the variety of loading time and cache performance of different browsers when visiting the same webpage, which has a great impact on the browsing experience. Furthermore, we try to find which metrics have significant effect on the differences, investigating the possible causes. Finally, according to our findings, we give some recommendations to web developers, browser vendors, and end users.

==> data.tex <==
%In this section, we have a brief introduction about the data collection, including the method and framework used to collect data and an overview of the data set.
In this section, we introduce our dataset and the experimental platform. Recalling the research questions that we are going to answer, we introduce the log traces of popular websites in first section. Then, we introduce the experimental environment and the framework of data collection.

\subsection{Page Visit Traces from Different Browsers }
The list of websites comes from Alexa~\cite{Alexa} top 500 ranking list. Each browser visits a part of it. We keep track of all request and response traffic for half a month. That is approximately 1400 visits for each webpage.

Considering some problems, we finally filtered out some of the following webpages:
\begin{itemize}
\item	Unreachable webpages. Some webpages are not available because of server internal error or network problem.
\item	Duplicate webpages. Some webpages have different domain names but actually offer the same service. We keep only one of them.
Finally, we have a data set of 334 webpages and 1000 visiting traces for each service. The total size is 4.6 terabytes. After parsing saved files, we have a database of over ten million records.
\end{itemize}
\subsection{Experimental Platform Setup}


To analyze the webpages on different browsers, we need a large quantity of empirical data collected in similar operating conditions except for browsers. Operating conditions, like computer hardware, operating system and network condition are controlled variables in our work. We carefully configured the environment to make sure that all these controlled variables doesn't influence the experimental results. We installed all browsers, Chrome, Firefox and Opera on several similar machines.

We carried out 24 groups of data collection at the same time: In 3 groups, we use Chrome, Firefox or Opera, to revisit a list of mobile websites every 30 minutes, with the cache of browsers disabled. In the other 21 groups, the browser cache is enabled, and the revisiting intervals are 30 minutes, 6 hours, 12 hours, 1 day, 2 days, 4 days and 7 days. We control to make sure that all these 24 groups visit a certain website simultaneously.

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{fig/framework}
\caption{The architecture of data collection.}
\end{figure}

Then we developed a set of tools to control all these browsers.

A visitor is a node requesting a webpage at a certain interval. The webpage is identified by a list of given URLs. A visitor is composed of three parts: a browser, an extension and a Charles web proxy~\cite{Charles}. Firstly we enable browsers` emulation mode and set the user agent to ``Android 4.2". In this case, the servers will return mobile-version services. When browsers render the web pages,more services are provided and finally a set of relevant resources will be loaded. Secondly, cache policy is set to be prohibited in browser configuration. Because we need to observe real traffic each time other than get the service from local cache.

Then, we use the Charles web proxy, a commercial product, to record all traffic during our visiting time. Charles records all TCP and HTTP/HTTPS connections pass through it. Moreover, Charles offers a set of APIs for programmers to access its data, which helps us download and save.

Finally, we build extensions for browsers to automatically revisiting a webpage. The extensions are a little bit different from each other because different browsers offer different interfaces for extensions. However, logic controls remain the same: all extensions are set to revisit a list of given URLs at a certain interval, then access data recorded in Charles and submit the response to collector. To make sure that a service has been loaded completely before shifting to the next one, we set a threshold of one minute. That`s to say, the second service will wait for at least one minute after the first service being requested.

We make sure that all visitors visit the same webpage at the same time within the same hardware and network environment.

A collector is a PHP server receiving all data collected by Charles and submitted by extensions. The PHP server receives data from all visitors and record information to local disk.

A central controller is used to control all the machines. It will set the starting time of data collection in order to make all browsers start their work simultaneously.  It can also stop or restart a certain browser to handle some exceptions during the work.




==> discussion.tex <==
In this section, we take discussion of some details in our work.

==> macros.tex <==
\newcommand{\code}[1]{\texttt{\footnotesize #1}}
\newcommand{\todo}[1]{{\color{red} \bf \{TODO: {#1}\}}}

\def\modify#1#2#3{{\small\underline{\sf{#1}}:} {\color{red}{\small #2}}
{{\color{red}\mbox{$\Rightarrow$}}} {\color{blue}{#3}}}
%\renewcommand{\modify}[3]{{#3}}

\newcommand{\lxmodify}[2]{\modify{Xuan}{#1}{#2}}

\newcommand\mymargin[1]{\marginpar{{\flushleft\textsc\footnotesize {#1}}}}
\newcommand\yxmargin[1]{\mymargin{XZ:\;#1}}

\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\eqnref}[1]{violation~\eqref{#1}}
\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\tblref}[1]{Table~\ref{#1}}
\newcommand{\smalltitle}[1]{{\smallskip \noindent \bf  {#1}.\ }}
\newcommand{\smalltitlecolon}[1]{{\smallskip \noindent \bf  {#1}:\ }}

\newtheorem{property}{Property}

\newcommand{\liumodifyok}[2]{#2}

\newcommand{\mycomment}[2]{{\small\color{magenta}\underline{\sf{#1}}:} {\color{magenta}{\small #2}}}
\newcommand{\xzlcomment}[1]{\mycomment{Xuanzhe}{#1}}
\newcommand{\liucomment}[2]{\mycomment{Xuan}{#2}}

% \renewcommand{\yxcomment}[1]{}
% \renewcommand{\yxmodify}[2]{#2}

==> metric.tex <==
In this session, we consider a list of factors that may be different in all browsers. Afterwards, we compare the importance of these factors and illustrate the major factors that cause difference on different browsers.
\subsection{Factors and metrics definition}
We consider several high-level factors of a certain website page. 
Scale of resources in a service may lead to different QoE on different browsers. Browsers may have their own strategies to parse and render a web page. Typically, the pre-fetching strategy may be suitable for services with large numbers of resources, because it saves the time for HTTP connection. On the other hand, it may cause redundant transmission for those services with few resources. 
Distribution of different types of resources may be influential. It includes the percentage of JavaScript, image, style sheet, HTML and JSON. Browsers may show different capabilities of handling these resources. For example, a browser that has better JavaScript parser may be suitable for services with a high proportion of JavaScript resources.
Dependence on third party services may have vital influences on QoE. It includes the percentage of third party services and the percentage of services specially provided by browsers. Browsers may show different preference to third-party services and even forbid some of the domains due to security reasons.
Redundant transmission can be different on different browsers. Redundant transmission consists of invalid resources with unexpected HTTP status code and duplicated resources. E.g., a resource responding with status 404 is invalid, and a resource having totally same URL with another one is duplicated. Redundant transmission may be caused by poor strategy of error handling. It varies among browsers.
Explicit cache control of resources in a Web-based service may influence the QoE in various ways. On one hand, a service with larger percentage of resources that have explicitly set cache methods will consume less traffic in the long term. On the other hand, cache policy may increase the response time and therefore worsen the performance. 
HTTPS secure mechanism offers extra security guarantee for users. However, HTTPS requires bidirectional encryption of communication and the capability of different browsers may be vary.
\begin{table}
\centering
\caption{FACTORS AND METRICS}
\begin{tabular}{|c|c|l|} 
\hline
Factors&Metrics&Comments\\ 
\hline
\multirow{2}{*} Scale of resources & Numbers of resources  &Size of resources  \\
\cline{2-3}
&Size of resources  &Total size of resources in a service. \\ 
\hline
$\pi$ & 1 in 5& Common in math\\ 
\hline
\$ & 4 in 5 & Used in business\\ 
\hline
$\Psi^2_1$ & 1 in 40,000& Unexplained usage\\
\hline\end{tabular}
\end{table}


\subsection{Results of RQ1: Difference of contents on different browsers}


==> multiple.tex <==




